Satisfaction relations for proper classes: Applications in logic and set theory

We develop the theory of partial satisfaction relations for structures that may be proper classes and define a satisfaction predicate appropriate to such structures. We indicate the utility of this theory as a framework for the development of the metatheory of first-order predicate logic and set theory, and we use it to prove that for any recursively enumerable extension T of ZF (Zermelo-Fraenkel set theory) there is a finitely axiomatizable extension T' of GB (von Neumann-Bernays-G\"odel class theory) that is a conservative extension of T. We also prove a conservative extension result that justifies the use of this predicate to characterize ground models for forcing constructions.

==> COLOR.tex <==
%%
%% This is file `color.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% color.dtx  (with options: `package')
%% 
%% color.dtx Copyright (C) 1994--1999 David Carlisle
%%
%% This file is part of the Standard LaTeX `Graphics Bundle'.
%% It may be distributed under the terms of the LaTeX Project Public
%% License, as described in lppl.txt in the base LaTeX distribution.
%% Either version 1.0 or, at your option, any later version.
%%
\NeedsTeXFormat{LaTeX2e}[1995/12/01]
\ProvidesPackage{color}
          [1999/02/16 v1.0i Standard LaTeX Color (DPC)]
\edef\Gin@codes{%
 \catcode`\noexpand\^^A\the\catcode`\^^A\relax
 \catcode`\noexpand\"\the\catcode`\"\relax
 \catcode`\noexpand\*\the\catcode`\*\relax
 \catcode`\noexpand\!\the\catcode`\!\relax
 \catcode`\noexpand\:\the\catcode`\:\relax}
\catcode`\^^A=\catcode`\%
\catcode`\"=12
\catcode`\*=11
\catcode`\!=12
\catcode`\:=12
\providecommand\Gin@driver{}
\def\c@lor@error#1{%
  \@latex@error{Undefined color #1}\@ehd}
\DeclareOption{monochrome}{%
  \def\c@lor@error#1{\PackageInfo{color}{Undefined color #1}}%
  \AtEndOfPackage{%
    \colors@false
    \def\set@color{%
      \c@lor@special\m@ne
        {color push \current@color}\aftergroup\reset@color}%
    \def\reset@color{\c@lor@special\m@ne{color pop}}%
    \def\set@page@color{%
      \c@lor@special\m@ne{background \current@color}}%
    \def\define@color#1#2{%
      \c@lor@special\m@ne{define #1 #2}}}}
\DeclareOption{debugshow}{\catcode`\^^A=9 \let\GDebug\typeout}
\DeclareOption{dvips}{\def\Gin@driver{dvips.def}%
                      \def\c@lor@namefile{dvipsnam.def}}
\DeclareOption{xdvi}{\ExecuteOptions{dvips,monochrome}}
\DeclareOption{dvipdf}{\def\Gin@driver{dvipdf.def}}
\DeclareOption{dvipdfm}{\def\Gin@driver{dvipdfm.def}}
\DeclareOption{pdftex}{\def\Gin@driver{pdftex.def}}
\DeclareOption{dvipsone}{\def\Gin@driver{dvipsone.def}}
\DeclareOption{dviwindo}{\ExecuteOptions{dvipsone}}
\DeclareOption{emtex}{\def\Gin@driver{emtex.def}}
\DeclareOption{dviwin}{\def\Gin@driver{dviwin.def}}
\DeclareOption{oztex}{\ExecuteOptions{dvips}}
\DeclareOption{textures}{\def\Gin@driver{textures.def}}
\DeclareOption{pctexps}{\def\Gin@driver{pctexps.def}}
\DeclareOption{pctexwin}{\def\Gin@driver{pctexwin.def}}
\DeclareOption{pctexhp}{\def\Gin@driver{pctexhp.def}}
\DeclareOption{pctex32}{\def\Gin@driver{pctex32.def}}
\DeclareOption{truetex}{\def\Gin@driver{truetex.def}}
\DeclareOption{tcidvi}{\def\Gin@driver{tcidvi.def}}
\DeclareOption{vtex}{\def\Gin@driver{vtex.def}}
\DeclareOption{dvipsnames}{\def\c@lor@namefile{dvipsnam.def}}
\DeclareOption{nodvipsnames}{\let\c@lor@namefile\relax}
\let\c@lor@usename\@gobble
\DeclareOption{usenames}{%
  \def\c@lor@usename#1{%
    \expandafter\color@named\csname\string\color @#1\endcsname{#1}}}
\DeclareRobustCommand\color{%
  \@ifnextchar[\@undeclaredcolor\@declaredcolor}
\def\@undeclaredcolor[#1]#2{%
  \@ifundefined{color@#1}%
    {\c@lor@error{model `#1'}}%
    {\csname color@#1\endcsname\current@color{#2}%
     \set@color}%
  \ignorespaces}
\def\@declaredcolor#1{%
  \@ifundefined{\string\color @#1}%
    {\c@lor@error{`#1'}}%
    {\expandafter\let\expandafter\current@color
     \csname\string\color @#1\endcsname
     \set@color}%
  \ignorespaces}
\def\textcolor#1#{\@textcolor{#1}}
\def\@textcolor#1#2#3{\protect\leavevmode{\color#1{#2}#3}}
\def\pagecolor{%
  \begingroup
      \let\ignorespaces\endgroup
      \let\set@color\set@page@color
      \color}
\def\definecolor#1#2#3{%
  \@ifundefined{color@#2}%
    {\c@lor@error{model `#2'}}%
    {\@ifundefined{\string\color @#1}{}%
      {\PackageInfo{color}{Redefining color #1}}%
     \csname color@#2\expandafter\endcsname
         \csname\string\color @#1\endcsname{#3}}}
\def\DefineNamedColor#1#2#3#4{%
  \@ifundefined{define@color@#1}%
    {\c@lor@error{model `#1'}}%
    {\@ifundefined{color@#3}%
      {\c@lor@error{model `#3'}}%
      {\@ifundefined{c@lor@#1@#2}{}%
        {\PackageInfo{color}{Redefining color #2 in named color model}}%
      \csname color@#3\endcsname\@tempa{#4}%
      \csname define@color@#1\endcsname{#2}\@tempa
      \c@lor@usename{#2}}}}
\@onlypreamble\DefineNamedColor
\newif\ifcolors@
\colors@true
\def\c@lor@special#1#2{%
  \edef\@tempa{\write#1{#2}}\@tempa}
\InputIfFileExists{color.cfg}{}{}
\ProcessOptions
\if!\Gin@driver!
  \PackageError{color}
    {No driver specified}
    {You should make a default driver option in a file \MessageBreak
     color.cfg\MessageBreak
     eg: \protect\ExecuteOptions{dvips}%
     }
\else
  \PackageInfo{color}{Driver file: \Gin@driver}
  \@ifundefined{ver@\Gin@driver}{\input{\Gin@driver}}{}
\fi
\@ifundefined{c@lor@namefile}{}{\input{\c@lor@namefile}}
\def\normalcolor{\let\current@color\default@color\set@color}
\AtBeginDocument{\let\default@color\current@color}
\def\color@block#1#2#3{%
  {\set@color\rlap{\ifcolors@\vrule\@width#1\@height#2\@depth#3\fi}}}
\def\colorbox#1#{\color@box{#1}}
\def\color@box#1#2{\color@b@x\relax{\color#1{#2}}}
\def\fcolorbox#1#{\color@fbox{#1}}
\def\color@fbox#1#2#3{%
  \color@b@x{\fboxsep\z@\color#1{#2}\fbox}{\color#1{#3}}}

\long\def\color@b@x#1#2#3{%
 \leavevmode
 \setbox\z@\hbox{\kern\fboxsep{\set@color#3}\kern\fboxsep}%
 \dimen@\ht\z@\advance\dimen@\fboxsep\ht\z@\dimen@
 \dimen@\dp\z@\advance\dimen@\fboxsep\dp\z@\dimen@
 {#1{#2\color@block{\wd\z@}{\ht\z@}{\dp\z@}%
      \box\z@}}}
\def\color@setgroup{\begingroup\set@color}
\let\color@begingroup\begingroup
\def\color@endgroup{\endgraf\endgroup}
\def\color@hbox{\hbox\bgroup\color@begingroup}
\def\color@vbox{\vbox\bgroup\color@begingroup}
\def\color@endbox{\color@endgroup\egroup}
\ifx\color@gray\@undefined
  \ifx\color@rgb\@undefined
  \else
    \definecolor{black}{rgb}{0,0,0}
    \definecolor{white}{rgb}{1,1,1}
  \fi
\else
  \definecolor{black}{gray}{0}
  \definecolor{white}{gray}{1}
\fi
\ifx\color@rgb\@undefined\else
  \definecolor{red}{rgb}{1,0,0}
  \definecolor{green}{rgb}{0,1,0}
  \definecolor{blue}{rgb}{0,0,1}
\fi
\ifx\color@cmyk\@undefined\else
  \definecolor{cyan}{cmyk}{1,0,0,0}
  \definecolor{magenta}{cmyk}{0,1,0,0}
  \definecolor{yellow}{cmyk}{0,0,1,0}
\fi
\Gin@codes
\let\Gin@codes\relax
\endinput
%%
%% End of file `color.sty'.

